Object-Centric Diagnosis of Visual Reasoning

When answering questions about an image, it not only needs knowing what -- understanding the fine-grained contents (e.g., objects, relationships) in the image, but also telling why -- reasoning over grounding visual cues to derive the answer for a question. Over the last few years, we have seen significant progress on visual question answering. Though impressive as the accuracy grows, it still lags behind to get knowing whether these models are undertaking grounding visual reasoning or just leveraging spurious correlations in the training data. Recently, a number of works have attempted to answer this question from perspectives such as grounding and robustness. However, most of them are either focusing on the language side or coarsely studying the pixel-level attention maps. In this paper, by leveraging the step-wise object grounding annotations provided in the GQA dataset, we first present a systematical object-centric diagnosis of visual reasoning on grounding and robustness, particularly on the vision side. According to the extensive comparisons across different models, we find that even models with high accuracy are not good at grounding objects precisely, nor robust to visual content perturbations. In contrast, symbolic and modular models have a relatively better grounding and robustness, though at the cost of accuracy. To reconcile these different aspects, we further develop a diagnostic model, namely Graph Reasoning Machine. Our model replaces purely symbolic visual representation with probabilistic scene graph and then applies teacher-forcing training for the visual reasoning module. The designed model improves the performance on all three metrics over the vanilla neural-symbolic model while inheriting the transparency. Further ablation studies suggest that this improvement is mainly due to more accurate image understanding and proper intermediate reasoning supervisions.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> texts/4-3-presupposition.tex <==
% \subsection{Question Relevance}
% \vspace{3pt}
%\vspace{-5pt}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/relevance.pdf}
%     \vspace{-20pt}
%     \caption{Three different type of questions From left to right, they are invalid, ambiguous, and answerable question.}
%     \vspace{-5pt}
%     \label{Figure:Relevance}
% \end{figure}
% \label{Sec:QuestionRelevance}
% \begin{table*}[t]
% \setlength{\tabcolsep}{3.3pt}
% \centering
% \begin{tabular}{l c c c c c c c c}
% \toprule
% Split & Bottom-Up~\cite{hudson2018compositional} & LCGN~\cite{hu2019language}  & LXMERT~\cite{tan2019lxmert} & NS-VQA~\cite{nsvqa} & MMN~\cite{chen2019meta} \\
% \midrule
%  Invalid       & 36.86     & 23.23     & \textbf{39.50}    & 34.77  & 0.56   \\
%  Ambiguous     & 31.90     & 37.28     & 3.16     & \textbf{61.39}  & 59.03  \\
%  Answerable    & 41.26     & 49.04     & 51.75    & 22.02  & \textbf{52.04}  \\
%  \midrule
%  All           & 36.73     & 40.71     & 29.62    & 41.19  & \textbf{48.02}  \\
% \bottomrule
% \end{tabular}
% \vspace{2pt}
% \caption{Question relevance classification result. The accuracies for each category and the full set are reported.}
% \label{Table:Relevance}
% \end{table*}

% In this section, we discuss the question relevance in the VQA task. In Ray~\etal\cite{ray2016question}, the authors proposed a method to identify the non-visual and false-premise questions by training a deep neural network to classify the questions. However, we argue that the ability to classify a question being answerable or not should be an automatically emerged feature when learning to answer the question; it should not require extra annotated data. In the GQA dataset, there is a noticeable number of questions that cannot be answered or have multiple (ambiguous) references or answers. 

% In this paper, we categorize questions into three types: 1) \textit{invalid}, which means that the question is totally not answerable; 2) \textit{answerable}, which means that a unique answer can be derived for it; 3) \textit{ambiguous}, which means that the question is answerable, but there are multiple references or answers to it. 
%e have assumed that the questions are always answerable on top of the given images. However, this does not necessarily happen n realistic scenarios. In this part, 
% We now delve into internal of visual reasoning to investigate whether visual reasoning models can determine the relevance between questions and images. On the GQA testdev set, we ask three AMT workers to annotate each question-image pair into one of the three types: invalid, ambiguous, and answerable. After taking the majority vote, we obtain 1,712, 5,149, and 5,695 question-image pairs that are labeled as invalid, ambiguous, and answerable, respectively. The high number of ambiguous instances indicate that many questions in the GQA testdev set are referring to multiple set of grounded objects. Intuitively, this might be caused by the incomplete scene graph annotations on the Visual Genome dataset~\cite{krishna2017visual} used by GQA.
% A few examples can be found in \fig{Figure:Relevance}.

% \xhdr{Metric.} To investigate whether the VQA models have an emerged ability to verify question relevance, we propose a heuristic method without any further re-training or fine-tuning steps. We rely on the object-oriented attention scores output from each model, considering that the question relevance correlates strongly with the existence of queried visual contents, and attention scores can be used as an indicator for this. Specifically, given a set of detected objects and their associated attention scores, we normalize and sort them in descending order. Based on the locations and attention scores, we then apply an NMS to filter boxes with an overlap larger than 0.5. Finally, we count the number of satisfied boxes by comparing their attention scores with a pre-determined threshold. If the number of satisfied boxes is 0, we predict the question as invalid; if it is larger than 1, we predict it as ambiguous; otherwise, we predict the question to be answerable. After we tune the threshold on the dev split, it turns out that this heuristic design works well for different methods. To make a fair comparison across different methods, we exhaustively tune the threshold on the testdev split, so that all methods achieve a balanced performance across three question types. This calibration is essential since the model can cheat by setting the threshold to 0 or 1 to predict all questions as ambiguous or invalid, respectively.
% Based on the annotations, we leverage the off-the-shelf models to classify question-image pairs into the three categories. We sample 3,000 question-image pairs from the full set for validation and use the remaining for testing. \tbl{Table:Relevance} shows the results. As we can see, overall MMN beats other models. However, the accuracies on three categories are not balanced though we exhaustively tried different hyper-parameters. Such issue also happens on LXMERT. In contrary. the other threes models achieve more balanced performance across three categories. Finally, we can see that the visual reasoning models can be directly transformed to a question relevance detector without any extra training data.

% We find that none of the methods may determine whether an question is answerable or not during test, except for NS-VQA++. With a similar accuracy on answerable questions, NS-VQA++ outperforms other methods on the other two question types. LXMERT~\cite{tan2019lxmert} has an extremely poor performance on \textit{ambiguous} question type, while MMN~\cite{chen2019meta} performs poorly on identifying invalid questions. These results are well correlated with our measures before: both LCGN and MMN fail in identifying invalid questions, as they can still make confident predictions based on irrelevant objects in the scene. LXMERT does not perform well in finding ambiguous questions, probably because it has been overfit to biases to resolve ambiguous questions during its pre-training phase.

==> texts/bak-0-abstract.tex <==
\begin{abstract}

Visual reasoning is a task not only about \textit{knowing what}, \ie, understanding the contents in question and image, but also about \textit{telling why}, \ie, reasoning over specific visual contents to derive the answer. Though significant improvements have been achieved in current visual reasoning models, most of them are heavily dependent on the correlations in training data. As such, they usually lack sufficient groundingness on the image contents and are vulnerable to subtle changes in the images or texts. In this paper, we leverage the fine-grained grounding annotations in GQA dataset and ask a fundamental question: What makes a good visual reasoning model? We argue that it should be not only accurate, but also interpretable, robust, and relevant to questions. An {\it interpretable} model should give answers based on the objects that the question refers to, but not other objects; a {\it robust} model should make consistent predictions when irrelevant objects are added to or removed from the image; a {\it question-relevant model} should be able to detect unanswerable or ambiguous questions. While most previous works have focused on improving the accuracy of VQA models, we present a systematic study of current VQA models beyond accuracy. We present new metrics and analyses to quantify the interpretability, robustness, and question relevance of these models, based on the representations they use for visual and textual input, as well as the way they perform reasoning. We find that using object-centric visual representations and program-like question representations improves the interpretability of the model. Incorporating symbolic execution of latent programs of questions makes models more robust and question-relevant.

%Visual Question Answering (VQA) is a task not only about \textit{knowing what}, \ie, understanding the contents in question and image, but also about \textit{telling why}, \ie, reasoning over specific visual contents to derive the answer. Though significant improvements have been achieved in current VQA models, most of them are heavily dependent on the correlations in training data. As such, they usually lack sufficient groundingness on the image contents and are vulnerable to subtle changes in the images or texts. 


% Old Abstract
% Visual Question Answering (VQA) is a task not only about \textit{knowing what}, \ie, understanding the contents in question and image, but also about \textit{telling why}, \ie, reasoning over specific visual contents to derive the answer. Though significant improvements have been achieved in current VQA models, most of them are heavily dependent on the correlations in training data. As such, they usually lack sufficient groundingness on the image contents and are vulnerable to subtle changes in the images or texts. \jw{not sure how "dependent on the correlations" leads to "lack sufficient groundingness". A model can depend on the correlations and at the same time have "groundingness"?} \jiayuan{I think the word is Groundedness?} In this paper, we take a step to encourage the model to perform grounded reasoning for visual question answering. By representing the image as a scene graph, we propose a new framework called Graph Reasoning Machine to enable an explicit \emph{and} grounded reasoning over the image contents. \jw{not sure if we should emphasize the model} \jw{before we talk about measures, it'd be important to explain what "groundingness" are necessary and important at the first place.} Moreover, we propose a method to quantitatively measure how much the models are grounded on the image contents, and how robust the models are to the modifications of irrelevant contents. In the experiments, we show that our model achieves comparable performance to other methods with much better groundingness and robustness. \jw{why talk about comparable performance?} Taking the merit of groundingness in our model, we further present a thorough analysis and diagnosis on what our model is and is not good at compared with other models. \jw{this is vague. any conclusions from the analysis?}  \jw{and it seems like we never mention robustness, presupposition in the abstract. Shall we?}
\keywords{Visual Question Answering, Visual Reasoning, Interpretability, Robustness, Question Relevance}
\end{abstract}

==> texts/bak-3-model.tex <==
\section{NS-VQA++}
% Motivation:  a strong human desire for explanations has not been sufficiently recognized by modern visual reasoning systems, in which most methods primarily focus on task performance.

% three merits: 1) the VQA task is disentangled into three sub-tasks, visual understanding, language understanding and reasoning, which can be tackled separately; 2) we can leverage the intermediate supervisions for each task whereas training the model end-to-end; 3) most importantly, the model becomes naturally \textit{interpretable} and \textit{explainable}. We can get a full understanding on how the model derives the answer and quickly diagnose each of the components.

% The reason for this choice is three-fold: 1) compared with feature level representation, semantic visual representations make the visual system output more interpretable and the errors can be easily back-progpagated to scene graph generator; 2) 

% Based on the above factorization, the proposed graph reasoning machine consists of three main components: a)  for $p(\bm{S}|\bm{I})$; b) Question Program Generator for $p(\bm{R}|\bm{Q})$; and c) Neural-Symbolic Executor for $p(\bm{a}|\bm{S}, \bm{R})$. 

\subsection{Scene Graph Generator}
\label{Sec:SceneGraph}
We use a scene graph $\bm{G}$ to represent the image considering that almost all visual questions mostly asking about objects, attributes or relationships.
% Recently, scene graph has been widely used and represented by either a group of features \cite{} or a set of pure symbols \cite{nsvqa}.
In this paper, we carefully design our own scene graph representation to facilitate the grounded reasoning in that: 1) it should be semantically meaningful for better interpretability; 2) it should be compatible with the reasoning module as well as gradient back-propagation. As such, we choose to use the classification scores output from scene graph generator to represent the scene graph. Specifically, a scene graph is denoted by $\bm{G} = <\bm{V},\bm{E}>$ where:
\begin{compactenum}[\hspace{5pt}1)]
\item $\bm{V}$ is a set of object proposals in the image. It contains $K = |\bm{V}|$ objects associated with bounding boxes $\bm{B} \in \mathcal{R}^{K \times 4}$, object classification scores $\bm{S_o} \in \mathcal{R}^{K \times {C}_o}$ and attribute classification scores $\bm{S_a} \in \mathcal{R}^{K \times C_a}$, where $C_o$ and $C_a$ are the number of object and attribute categories, respectively. Both contain the background class.
\item $\bm{E}$ is the set of edges connecting the objects in the scene graph. Each edge is associated with a predicate classification score. Here, we cover all object pairs in the image to construct a score matrix $\bm{S}_p \in \mathcal{R}^{K \times K \times C_p}$, where $C_p$ is the number of predicate categories including background class.
\end{compactenum}

To extract the above scene graph representation, we extend the method proposed in \cite{yang2018graph} and \cite{zellers2018neural} by adding an attribute classification module for each object proposal. Specifically, given the object proposals $\bm{B}$ and the corresponding features $\bm{X}_o = \{\bm{x}_o^i\}$, we have three modules $\{\mathrm{\Phi}_{o}, \mathrm{\Phi}_{a}, \mathrm{\Phi}_{p}\}$ to predict $\bm{S}_o$, $\bm{S}_a$ and $\bm{S}_p$, respectively:
\begin{equation}
    \bm{S}_o = \mathrm{\Phi}_{o}(\bm{X}_o); \quad \bm{S}_a = \mathrm{\Phi}_{a}(\bm{X}_o); \quad \bm{S}_p = \mathrm{\Phi}_{p}(\bm{X}_o)
\end{equation}

Note that these scores $\bm{S}_o$, $\bm{S}_a$ and $\bm{S}_p$ are the logits before softmax layers since it contains the same semantic information as probability distribution while facilitating the gradient back propagation from upper layers to lower layers. 
% More detailed description can be found in our experimental section. 

\subsection{Program Generator}

To enable explicit reasoning, we use a program generator to extract the reasoning programs from questions. Each program consists of several operators and each operation consists of three components:
\begin{compactenum}[\hspace{5pt}1)]
\item \textbf{Operator}. It is the logic skeleton in the program. To cover diverse questions in GQA dataset, we introduce 10 different operators, including \textit{filter}, \textit{query}, \textit{exist}, \textit{verify}, \textit{common}, \textit{relate}, \textit{choose}, \textit{and}, \textit{or}, \textit{not};
\item \textbf{Concept}. This is used to specify the super category for the operator. For different operators, it has different options. For example, for \textit{filter}, the concept can be object concept (\eg, person, animal, furniture), attribute concept (\eg, color, material) or position concept (\eg, vertical position); for \textit{relate}, it can be subject or object;
\item \textbf{Category}. This is the most fine-grained argument in the program, and is also determined by the concept in the program. For example, if the object concept is \textit{animal}, then the category can be dog, sheep, cow, \etc.
\end{compactenum}

Based on above hierarchical combination, we have in total 7445 different operations. A full description of operations can be found in our supplementary material. For each question, we can build a unique reasoning program by connecting the operations under the dependency constraint. For example, the question ``How large is the white boat?" can be converted to a reasoning program ``filter(boat)-filter(white)-query(size)''.

A program generator is aimed at converting a raw question $\bm{Q} = \{{q}_1, ... , {q}_T\}$ to a reasoning program with $K$ operations $\bm{R} = \{{r}_1, ... , {r}_K\}$. Here, we use a simple sequence to sequence architecture. Specifically, given a question $\bm{Q} = \{{q}_1, ... , {q}_T\}$, we fist use an embedding layer to encode each word ${q}_i$ to a vector $\bm{x}_q^i$. Then, we feed the sequence of word embeddings into a bidirectional LSTM to obtain the representation for the whole question: $\{\bm{e}_f, \bm{e}_b\} = \mathrm{BiLSTM}(\{\bm{x}_q^{1:T}\})$, where $\bm{e}_f$ and $\bm{e}_b$ are the outputs of LSTM in forward and backward direction, respectively. These two embeddings are concatenated and used as the initial hidden state $\bm{h}^0_r = [\bm{e}_f | \bm{e}_b]$ to another LSTM to derive the reasoning program:
\begin{equation}
    \bm{h}_r^i = \mathrm{LSTM}(\bm{x}_r^i, \bm{h}_r^{i-1}); \quad  y_r^i \sim \mathrm{Softmax}(\bm{W}^T \bm{h}_r^i) \\
\end{equation}
where $\bm{x}^i_r$ is the embedding vector for the input operation token at $i$-th step; $y^i_r$ is the output operation token at $i$-th step which is sampled by sending the hidden state $\bm{h}_r^i$ to a fully-connected layer with parameter $\bm{W}^T$. At training and test time, $\bm{x}^i_r$ is the embedding for the ground-truth token and predicted token from last step, respectively. The output dimension of embedding layer for both question and operation tokens are 300. Though simple enough, it turns out that our program generator can achieve almost perfect performance, with over 95\% prediction accuracy on the validation set. This decent program generation is the basis for us to perform grounded reasoning.

\subsection{Neural Executor}

After obtaining the scene graph and reasoning program, we execute the program on top of the scene graph to derive the answer. For VQA on realistic images, we find a conventional symbolic executor (\ie, \cite{nsvqa}) does not work well due to the defective visual system on realistic images. To mitigate this problem, we propose a neural executor which can be learnable and differential with respect to the semantic visual representation.

In neural executor, executing a reasoning program $\bm{R}$ is a process of traversing on the scene graph $\bm{G}$ along the logic chain until we get the answer. At a high level, there are three type of operations. The first type is pointing operation such as \textit{filter}, \textit{relate}, whose inputs and output are both a set of indices. The second type is binary operation whose output is a scalar score indicating a Boolean decision, such as \textit{exist} and \textit{verify}. The last one is the ending operation which outputs the final answer to a question. In the following, we will explain how they are implemented in our neural executor.

\begin{table}[t]\footnotesize
\setlength{\tabcolsep}{5.3pt}
\centering
\begin{tabular}{l c c c c}
\toprule
Operator & Concept & Category & Inputs & Outputs  \\
\midrule
\textit{filter} & $\{obj, attr\}$ & $\in {V}_{\{o, a\}}$ & $[\bm{n_i}]$ & $[\bm{n_o}]$ \\
\textit{relate} & $\{subj, obj, attr\}$ & $\in {V}_p$ & $[\bm{n^s_i}, \bm{n^o_i}]$ & $[\bm{n_o}]$\\
\textit{common} & $attr$ & - & Symbolic & attribute concept \\
\textit{query}  & $\{obj, attr\}$ & - & \\
\textit{exist}  & - & - & \\
\textit{verify} & & & \\
\bottomrule
\end{tabular}
\caption{Arguments for different operations.}
\label{Table:ReasoningOperation}
\vspace{-10pt}
\end{table}

\xhdr{Pointing Operation}. Executing a pointing operation can be thought as a process of referring expression. Given a set of candidates regions in the scene graph, the goal is to find the target regions which satisfy the arguments in the operation. For example, given an operation $filter(color(yellow))$, executor will specifically search for the objects with yellow color from the candidate pool, and output a new set of regions. Formally, for an pointing operation $\bm{r}$, its inputs contain: 1) $m$ index sets $\bm{Z} = \{\bm{z}_1, ..., \bm{z}_m\}$, where the $i$-th index set $\bm{z}_i=\{z_i[1],...,z_i[n]\}$ contains $n$ indices; 2) the corresponding score $\bm{A} = \{\bm{a}_1,...,\bm{a}_{m}\}$ associated with each index in $\bm{Z}$ and 3) the scene graph $\bm{G}$. After the execution, it outputs a new set of indices and scores:
\begin{equation}
    \{\bm{Z}^i, \bm{A}^i\} = \mathrm{executor}[\bm{r}^i](\bm{Z}^{i-1}, \bm{A}^{i-1}, \bm{G})
\end{equation}
where $\mathrm{executor}[\bm{r}^i]$ is the execution module corresponding to operation $\bm{r}^i$. For all pointing operations, the number of input sets is 1 or 2 depending on the type of operations (\eg, $m=1$ for \textit{filter} and $m=2$ for \textit{relate}), while the number of output sets is always 1. Inside the execution module, the selection of target regions is implemented by learning a scoring function on the input regions. In the following we will introduce two pointing operations \textit{filter} and \textit{relate}.

For the \textit{filter} operation, the executor takes as inputs the candidate object indices $\bm{z}^{i-1}$ and corresponding scores $\bm{a}^{i-1}$. The scores on the candidate regions are then calculated by:
\begin{equation}
    \bm{p}^i = (1 - \alpha) \bm{a}^{i-1} + \alpha \left(\hat{\bm{S}}^c_l \circ \sigma(\psi(\hat{\bm{B}})) \right)
    \label{Eq:intermediateOperation}
\end{equation}
where $\hat{\bm{S}}^c_l \in \mathcal{R}^{|\bm{z}^{i-1}| \times 1}, l \in \{o, a\}$ is a slice of the object/attribute score matrix according to the queried concept $l$, corresponding category index $c$ and the input object indices $\bm{z}^{i-1}$; $\hat{\bm{B}}$ is the bounding boxes at indices $\bm{z}^{i-1}$; $\psi(\cdot)$ and $\sigma(\cdot)$ are a non-linear function and sigmoid function, respectively; $\circ$ is the component-wise multiplication. Eq.~\eqref{Eq:intermediateOperation} ensures that the reasoning is always grounded on the scene graph entries specified by the arguments in operation. Simultaneously, we introduce a non-linear layer to learn to modulate the scores with object locations for a better groudingness. Finally, we sum up the resulting scores with scores from last step $\bm{a}^{i-1}$ with a weight $\alpha$ to obtain the final scores $\bm{p}^i$. Before moving to the next operation, we choose the top-ranked entries in $\bm{p}^i$ to compose $\{\bm{z}^i, \bm{a}^i\}$.

For \textit{relate} operation, we have two input index sets $\{\bm{z}_1, \bm{z}_2\}$ and scores $\{\bm{a}_1,\bm{a}_2\}$ for subject and object, respectively. The goal is to select the target regions from $\bm{z}_2$ using the following scoring function:
\begin{equation}
    \bm{p}^i = (1 - \alpha) \bm{a}^{i-1}_{2} + \alpha \left<\hat{\bm{S}}_p^c \circ \sigma(\psi(\hat{\bm{B}}_1) \phi(\hat{\bm{B}}_2)^T), \hat{\bm{a}}^{i-1}_{1}\right>
\end{equation}
where $\hat{\bm{S}}_p^c \in \mathcal{R}^{|\bm{z}_1^{i-1}| \times |\bm{z}_2^{i-1}|}$ is the sub-matrix of predicate score matrix according to input indices $\{\bm{z}_1, \bm{z}_2\}$ and predicate category $c$; $\psi$ and $\phi$ are two non-linear function to encode the object locations; $\hat{\bm{a}}_1^{i-1}$ is the normalized scores after passing ${\bm{a}}_1^{i-1}$ to softmax, which is then used to average the scores over dimension $\bm{z}_1$. Similarly, we take the top-ranked indices from the input indices according to $\bm{p}^i$ and compose the $\{\bm{z}^i, \bm{a}^i\}$ for the next operation.

\xhdr{Binary Operation}. Unlike pointing operations, scoring operation such as \textit{exist} does not output any target indices. Instead, it outputs a scalar score. Take \textit{exist} operation as an example. We take the maximum score in the input scores $\bm{a}^{i-1}$ and then pass it to a one-dimensional linear layer to calibrating its value range, ${p}^i = w \cdot \max(\bm{a}^{i-1}) + b$. Similarly, a \textit{verify} operation also use an one-dimensional linear layer to calculate the output score:
\begin{equation}
    p^i_l = w_l <\hat{\bm{S}}^c_l, \bar{\bm{a}}^{i-1}> + b_l
    \label{Eq:BinaryOperation}
\end{equation}

Depending on the specific reasoning program, scoring operation can be either an intermediate operation or an operation output the final answer. When it is an intermediate operation, its output score will be sent to the operations merely taking scores as input, such as \textit{and}, \textit{or}, \textit{not}. 

\xhdr{Ending Operation}. Ending operation is aimed at output the final answer to the question. We take \textit{query} as the example. Given  the input indices and scores $\{\bm{z}^{i-1}, \bm{a}^{i-1}\}$, the output scores for a query operation is:
\begin{equation}
    \bm{p}^i_l = (\hat{\bm{a}}^{i-1})^T (\hat{\bm{S}}_l \circ \sigma(\psi(\hat{\bm{B}}))
    \label{Eq:FinalOperation}
\end{equation}

Similar to Eq.~\eqref{Eq:intermediateOperation}, $l \in \{o, a\}$ is the concept specified in the \textit{query} operation; $\hat{\bm{S}}_l \in \mathcal{R}^{|\bm{z}^{i-1}| \times C_{l}}$ is the score matrix for object indices $\bm{z}^{i-1}$. Passing $\bm{p}^i_l \in \mathcal{R}^{1 \times C_l}$ into a softmax layer, we can obtain the probability distribution over all object or attribute categories and then give the final answer. Besides \textit{query}, the aforementioned binary operations such as \textit{verify}, \textit{exist} can be also ending operations. When working as an ending operation, they convert the score into a Boolean output `yes' or `no' as the final answer.

Due to the limited space, we briefly summarize all the operations in Table~\ref{Table:ReasoningOperation}. A more detailed description can be found in our supplementary material. For all the starting operations in a reasoning program, the input indices are all the object nodes, \ie, $\bm{z}^0 = \{1, ..., K\}$ and the scores are all 0, \ie, $\bm{a}^0 = \bm{0}^{K \times 1}$.

\xhdr{Teacher-forcing Training}. In our neural executor, we care about not only the correctness of final answer, but also the groundingness of each operation in the reasoning program. Motivated by this, we introduce a teacher-forcing training strategy, which simultaneously supervise the outputs of intermediate operations and the prediction of final answer.

To collect the supervisions for training our neural executor, we use the ground-truth scene graphs and reasoning programs provided in the training data. Given the ground-truth scene graph $\bm{G}^{gt}$ which is composed of symbolic category annotations, we run the ground-truth program $\bm{R}^{gt}$ on it. Through such a purely symbolic reasoning, we can obtain the selected indices for all pointing operations, Boolean values for all binary operations and the answers for the ending operations. This step-wise knowledge enable us to learn the parameters in our neural executor like a sequence generation model. In the following, we will elaborate how we compute the loss for each type of operation:
\begin{compactenum}[\hspace{5pt}1)]
\item \textit{Pointing operation}. Assume we have the ground-truth input indices $\{\bm{z}^{gt}_{i-1}\}$ and corresponding boxes $\bm{B}^{gt}_{i-1}$ in the ground-truth scene graph. We first compute the IoUs between detected boxes $\bm{B}$ and $\bm{B}^{gt}_{i-1}$. Then we find the indices $\bm{z}^{i-1}$ of boxes in $\bm{B}$ which have IoU$>0.5$ with any in $\bm{B}^{gt}_{i-1}$. These indices along with the scores $\bm{a}^{i-1}$ are then used to compute the pointing score $\bm{p}_l^i$ as in Eq.~\eqref{Eq:intermediateOperation}. Likewise, we find the matched indices in $\bm{B}$ with the ground-truth output $\bm{B}^{gt}_{i}$. Given the input indices $\bm{z}^{i-1}$ and output indices $\bm{z}^{i}$, we generate binary labels $\bm{y}^i$ of same size with $\bm{z}^{i-1}$ indicating whether the index is contained in $\bm{z}^{i}$. Then, we pass $\bm{p}^i$ to a sigmoid function and minimize the binary cross entropy between it and $\bm{y}^i$. This will help to push the operation to select the correct subset of regions from the inputs. Along with the ground-truth indices, the corresponding subset of scores in $\bm{p}^i$ are also sent to the next operation.

\item \textit{Binary operation}. Given the scores from last operation, we compute the output score $p_l^i$ using Eq.~\eqref{Eq:BinaryOperation}, and then use it to compute the binary cross entropy loss with the ground-truth Boolean label.

\item \textit{Ending operation}. Similar to pointing operation, we first find the highly-overlapped bounding boxes in $\bm{B}$ given $\bm{B}^{gt}_{i-1}$ as well as the corresponding scores from last operation. Then we use Eq.~\eqref{Eq:FinalOperation} to compute the probability over all candidate answers and compute a cross-entropy loss to the ground-truth answer.
\end{compactenum}

% During the training time, we have the ground-truth scene graph $\bm{S}^{gt}$ and reasoning programs $\bm{R}^{gt}$. We make use of these annotations to enforcing the output of each operation in the reasoning match the ground-truth output. This strong supervision turns out help a lot for the training of our reasoning module.

\xhdr{Inference}. During inference, we run the executor given the predicted scene graph and program. We introduce a beam search strategy to derive the final answer. At each pointing operation, we select the top $m$ choices in the outputs and then pass them to the next operation. This way we can obtain a global score in the ending operation which aggregate the predictions from all previous operations. We find in our experiments that such search strategy is slightly better than the greedy counterpart.

\subsection{Implementations Details}

\xhdr{Scene graph generator.} We use ResNeXt-101 \cite{xie2017aggregated} as its backbone and Faster R-CNN \cite{ren2015faster} to detect objects from images. For attribute classification, we reuse the box features from object detector and add a single MLP layer to predict the attribute scores. For relationship detection between objects, we use Graph R-CNN \cite{yang2018graph} and freq-prior knowledge \cite{zellers2018neural} to obtain the relationship scores for all object pairs in an image. To ensure the output vocabulary in our scene graph match those in the questions and programs, we collect 1702 object categories, XXX attribute categories and XXX relationship categories in the training set. We train our scene graph generator for 150k iterations use stochastic gradient descent (SGD) with learning rate 5e-3, batch size 8, momentum 0.99, and weight decay 5e-4. We reduce the learning rate by factor 10 at iteration 100k and 120k.

\xhdr{Program generator.} As mentioned earlier, we use a sequence-to-sequence model to implement the program generator. On the encoder side, we use a two layer bi-directional LSTM with hidden size 256. For decoder, we use a two-layer LSTM with hidden size 512. The vocabulary sizes for encoder and decoder are 2981 and 7445, respectively. We train it using Adam optimizer \cite{kingma2014adam} with learning rate 1e-3 for 70k iteration with batch size 256.

\xhdr{Join training.}
As discussed above, the disentanglement in our model make it possible to train each component separately. In this paper, the model is trained in three stages: 1) scene graph generator training, 2) program generator training, and 3) joint training of the scene graph generator and the neural executor.

During the joint training phase, we use the pretrained scene graph generator to detect objects from images, followed a non-maximum-suppression (NMS) to filter highly overlapped boxes. The resulting scene graph scores are then fed to neural executor. Fixing the backbone and feature extraction layers in scene graph generator, we train the neural executor as well as the classification layers in scene graph generator jointly for 100k iterations using SGD with learning rate 1e-3, batch size 8, momentum 0.99, and weight decay 5e-4. We reduce the learning rate by factor 10 at iteration 70k and 90k.


% \section{Diagnoses and Discussions}

% \begin{table}[t]\footnotesize
% \setlength{\tabcolsep}{3.2pt}
% \centering
% \begin{tabular}{l c c c c c c c c}
% \toprule
%               & gt-sg & gt-rel & gt-obj & gt-att & w/ cnn-lstm &  \\
% \midrule
% accuracy       & -     & -     & -     & -     & -     \\
% groundingness  & -     & -     & -     & -     & -     \\
% robustness     & -     & -     & -     & -     & -     \\
% \bottomrule
% \end{tabular}
% \vspace{5pt}
% \caption{Comparing groundingness across different methods.}
% \label{Table:Groundingness}
% \vspace{-10pt}
% \end{table}

% Though our proposed model has the ability to perform more grounding reasoning, a question to ask here is why our model cannot beat the other models. In this section, we explore the possible reasons to explain why our model cannot achieve state-of-the-art performance though equipped with some good properties as discussed above.

% Visual understanding is not good enough.

% \xhdr{replace detected scene graph with ground-truth scene graph}

% \xhdr{replace detected relationship with ground-truth relationship}

% \xhdr{simply train another LSTM model and add such language priors to our model to see whether the performance will be improved}



==> texts/bak-4-analysis.tex <==
\section{Model Dissection}

\begin{figure}[t]
    \centering
  	\includegraphics[height=3cm]{figures/groundingness/grounding-1.png}
    \caption{place holder for model dissection.}
    \label{fig:model-dissection}%
\end{figure}

To understand VQA models, it is important to make a dissection on them beyond reporting the accuracy. Before going details, we first define \emph{grounded objects} as a set of ground-truth objects on which the VQA models should be grounded to answer the question. We then categorize those detected objects which have a high overlap with the grounded objects as \emph{relevant objects}; otherwise as \emph{irrelevant objects}. As shown in Fig.~\ref{fig:model-dissection}, to answer the question ``What is on the bike that is on the stone?'', the grounded objects are labeled as green bounding boxes including ``bike'', ``stone'' and ``seat''. In the following, we present methods to dissect VQA models from three aspects:

\xhdr{Groundingness}. The key target of this paper is enable VQA model to perform grounded reasoning. Despite groundingness has been thought as an important property in VQA models in the community, no one has provided a way to quantify it. In this paper, we propose a new metric to \emph{quantitatively} measure it for various VQA models.

As shown in Fig.~\ref{fig:model-dissection}, given an image and a question, we first find the grounded objects $\{b_i\}$ from the image regarding the specific question. Then we run a VQA model on the inputs and then get the attention score for each detected objects from the image.

\xhdr{Robustness}. A grounded VQA model should be robust to modifications to the irrelevant image contents. Inspired by the work in \cite{Agarwal2019TowardsCV}, we further measure the model robustness to verify how sensitive the VQA models are to modifications on irrelevant image contents. However, different from \cite{Agarwal2019TowardsCV} which directly modify the pixels of a region in an image, we propose a more semantic modification by manipulating the existence of irrelevant objects. Through erasing, adding or perturbing the features of irrelevant objects in the image, we can have a sophisticated controlling on the presence of irrelevant objects, while ensuring the relevant objects not being modified.

Given the relevant objects 

\xhdr{Presupposition}. 

% \xhdr{Question Relevance}. 
